VioPose: Violin Performance 4D Pose Estimation by Hierarchical Audiovisual Inference

Musicians delicately control their bodies to generate music. Sometimes, their motions are too subtle to be captured by the human eye. To analyze how they move to produce the music, we need to estimate precise 4D human pose (3D pose over time). However, current state-of-the-art (SoTA) visual pose estimation algorithms struggle to produce accurate monocular 4D poses because of occlusions, partial views, and human-object interactions. They are limited by the viewing angle, pixel density, and sampling rate of the cameras and fail to estimate fast and subtle movements, such as in the musical effect of vibrato. We leverage the direct causal relationship between the music produced and the human motions creating them to address these challenges. We propose VioPose: a novel multimodal network that hierarchically estimates dynamics. High-level features are cascaded to low-level features and integrated into Bayesian updates. Our architecture is shown to produce accurate pose sequences, facilitating precise motion analysis, and outperforms SoTA. As part of this work, we collected the largest and the most diverse calibrated violin-playing dataset, including video, sound, and 3D motion capture poses. Code and dataset can be found in our project page \url{https://sj-yoo.info/viopose/}.

==> sec/6_sup.tex <==
\onecolumn
\section{Implementation Details}
\subsection{Loss Function}
Our loss function consists of three losses: the final pose estimation loss $\mathcal{L}_{P}$, the audio-to-pose loss (P2A loss) $\mathcal{L}_{A}$, and the cycle loss $\mathcal{L}_{C}$.  
The pose estimation loss $\mathcal{L}_{P}$ is defined using the MPJPE (Mean Per Joint Position Error), MPJVE (Mean Per Joint Velocity Error), and MPJAE (Mean Per Joint Acceleration Error) as follows:
\begin{align}
    \mathcal{L}_{P} = \lambda_{P_1}\text{MPJPE} + \lambda_{P_2} \text{MPJVE} + \lambda_{P_3}\text{MPJAE} 
\end{align}
where we used $\lambda_{P_1}=0.85, \lambda_{P_2}=0.1, \lambda_{P_3}=0.15$ as balancing weights.
$\mathcal{L}_{A}$ is defined by the  MPJPE. The cycle loss, $\mathcal{L}_{C}$, is defined by the $\mathrm{L}_{2}$ distance between the ground truth tempogram and the estimated tempogram.
Our final loss function amounts to 
\begin{align}
    \mathcal{L} = \mathcal{L}_{P} + \lambda_{A} \mathcal{L}_{A} + \lambda_{C}\mathcal{L}_{C}
\end{align}
where $\lambda_{A,C}$ are balancing weights and we used 0.15 and 20, respectively. 
The definition of MPJPE, MPJVE, and MPJAE is as follows:

\begin{equation}
\begin{split}
    &\mathcal{L}_{P} = \lambda_{P_1}\text{MPJPE} + \lambda_{P_2} \text{MPJVE} + \lambda_{P_3}\text{MPJAE} \\ 
    &\text{MPJPE}(p_k, p_{k}^{GT}) = \frac{1}{J} \sum_{j=1}^{J} || p_{k}-p_{k}^{GT}||_{2} \\ 
    &\text{MPJVE}(p_k, p_{k}^{GT}) = \frac{1}{J} \sum_{j=1}^{J} || \dot{p}_{k}- \dot{p}_{k}^{GT}||_{2} \\ 
    &\text{MPJAE}(p_k, p_{k}^{GT}) = \frac{1}{J} \sum_{j=1}^{J} || \ddot{p}_{k}-\ddot{p_{k}}^{GT}||_{2}
\end{split}
\end{equation}
where $p_{k}$ and $p_{k}^{GT}$ are the $k$-th estimated 3D joint and its ground truth, respectively. MPJVE and MPJAE  help the generated motions follow ground truth trajectories, the effect of the MPJVE and MPJAE loss terms are shown in Table~\ref{tab:abl_loss}. 


\begin{table}[b]
    \caption{\textcolor{blue}{Ablation study of effect of loss function and different architecture. We set pose estimation loss ($\mathcal{L}_P$) only with MPJPE (second row). The last row shows the result of replacing spatial transformer to temporal transformer}} 
    \centering
    \begin{tabular}{l |c|c|c}
        \Xhline{1pt}
        \textbf{Method}& \textbf{MPJPE} $\downarrow$ & \textbf{P-MPJPE} $\downarrow$  & \textbf{MPJAE} $\downarrow$ \\
        \hline
        Baseline & \textbf{44.03} &	\textbf{25.99} &	\textbf{1.59} \\
        $\mathcal{L}_{P_2}=\mathcal{L}_{P_3}=0$  &44.92 &	25.72 &	1.69\\
        $\mathcal{L}_{P_3}=0$  &45.53 &	26.01 &	1.71\\
        Temporal Transforme & 46.21 &	26.45 &	1.60 \\ 
        \Xhline{1pt}
    \end{tabular}
    \label{tab:abl_loss}
\end{table}

\subsection{Implementation Details of SoTA}
\textcolor{blue}{We retrained all the models with \DataName. To directly compare with proposed algorithm, we modified the total number of final output keypoints as eight, which is the only upper body joints. We chose the best-scored model and followed the instructions from their GitHub and paper. }

\paragraph{PoseFormerV2}~\cite{zhaoPoseFormerV2ExploringFrequency2023} \textcolor{blue}{We trained the model with 3 central frames, 3 Discrete Cosine Transform (DCT) coefficients on 81-frame sequences with 4 Transformer blocks, a hidden dimension of 32, across 200 epochs, and a learning rate of 0.0001 with a shrink factor of 0.99 for every epoch.} 

\paragraph{STCFormer}~\cite{tang3DHumanPose2023} \textcolor{blue}{We trained the model with 81 input sequence length, 6 layers, 256 hidden embedding channel, and the number of head 8, across 80 epochs and using a learning rate of 0.01 with a shrink factor of 0.96 for every epoch. Specially, STCFormer directly utilize the body structure, we modified total body group as number of two (left and right arm). }

\paragraph{MixSTE}~\cite{zhangMixSTESeq2seqMixed2022} \textcolor{blue}{We trained the model with 243 input sequence length, 8 spatial and temporal Transformer layers (same as the number of loops), embedding dimension of 512, and MLP hidden dimension of 1024, across 120 epochs and using a learning rate of 0.00004 with a shrink factor of 0.99 for every epoch.} 



\section{Details of \ITW \ data}
To evaluate generalization, we carefully collected \ITW \ data. This data  was collected from 6 participants (none of them are in the \DataName) of different genders, heights, violin skills, and wearing everyday clothing. Furthermore, we set up a room environment with multiple objects (i.e., sofa, table, chairs, books, purse, jackets, and plants), which were not included in \DataName. For evaluation, we used a markerless motion capture system with 8 different cameras. Note that \DataName \ was recorded using a marker-based motion capture system. We used one mobile phone placed next to one of the 8 reference cameras to record sound, and generated \ITW \ with this reference camera and the audio as shown in Fig.~\ref{fig:wild}. The values recorded from the markerless system are used as ground truth for us to provide P-MPJPE and P-MPJAE values.

\section{Further Experimental Results}
\subsection{Tempogram Estimation Results}
Figure ~\ref{fig:tempo} presents the estimated tempogram alongside its ground truth, derived from 3D pose output. The accuracy of the tempogram is fundamentally linked to the representation of the right arm's bowing motion. If the bowing trajectories are inaccurately generated, the cycle loss increases. The process of pose-to-audio generation bears similarities to motion translation, albeit into a different modality.

\subsection{Further Ablation Study} Our exploration into the ablation study of the loss function revealed that the MPJPE and MPJAE loss terms play a crucial role in the reduction of all evaluated metrics. Additionally, we experimented with substituting the spatial transformer, which focuses on body structure embedding, for a temporal transformer that prioritizes temporal information over structural details of the body. The findings underscore the importance of initially extracting body structural information.

\begin{table}[t]
    \caption{\textcolor{blue}{Ablation study of effect of input sequence length. We fixed the sampling rate of audio feature as 100 and varied input sequence time to one second, three second (baseline), and four second. The longer input sequence we use, the better MPJAE we achieved. However, the overall performance is the best when we use three second sequence as input.}} 
    \centering
    \begin{tabular}{l |c|c|c}
        \Xhline{1pt}
        \textbf{Method}& \textbf{MPJPE} $\downarrow$ & \textbf{P-MPJPE} $\downarrow$  & \textbf{MPJAE} $\downarrow$ \\
        \hline
        T=30 & 45.73	&26.20&	2.81 \\
        T=60 & 44.90 & \textbf{25.42} & 1.88 \\
        T=90 (Baseline) &\textbf{44.46} &	{25.49} &	1.59\\
        T=120  &45.75 &	25.83&	\textbf{1.48}\\
        \Xhline{1pt}
    \end{tabular}
    \label{tab:abl_loss}
\end{table}

\subsection{Qualitative Results}
\textcolor{blue}{We qualitatively evaluate the proposed algorithm with other SoTA methods in various ways. Note that we only trained models with train data of \DataName \ and tested on test data of \DataName, \ITW, and YouTube videos.}

\textcolor{blue}{We generate right wrist trajectories after Procrustes projection from the test set of \DataName \ within three-second windows, as illustrated in Fig. ~\ref{fig:trajectory}. Analyzing these trajectories is essential for understanding the violin bowing motion. Generally, \AlgName \ achieves superior estimations, particularly, in cases of rapid movements (rows 4 and 6 in Fig. ~\ref{fig:trajectory}). Moreover, violin bowing trajectories contain wide range of motion, from large movements\textemdash approximately 400 mm in the first row of figure\textemdash to subtle movements, with a range of motion less than 50 mm in the last row of figure. Other architectures, including \AlgName \ without audio model, fail to accurately capture these movements. Note that the slight offsets of trajectories are caused by the accumulation of errors after Procrustes projection. Fig~\ref{fig:viodat_rsult} presents qualitative results tested on \DataName \ in one-second intervals. At the frame level, some models estimate better than others. However, examining continuous trajectories reveals that the estimations lead to significantly different outcomes, which affect downstream task accuracy.}

\textcolor{blue}{We present pose estimation results from a random YouTube video as shown in Fig.~\ref{fig:youtube_2} and Fig.~\ref{fig:youtube_1}. Fig.~\ref{fig:youtube_2} shows the effectiveness of the audio module. Without an audio module, the architecture fails to track dynamics, which could cause the deterioration of downstream tasks.}

\subsection{Failure Cases}
\textcolor{blue}{While \AlgName \ proposes significant improvement thanks to additional information from audio, we have identified some failure cases that need improvement in future work. }

\textcolor{blue}{The first case involves \AlgName's difficulty in capturing vibrato movements, as illustrated in Fig.~\ref{fig:Vibrato}. Vibrato is a crucial musical technique and serves as a tool for musicians to express emotions. However, its subtle and limited range of motion impedes accurate pose estimation. Capturing such movements based solely on visual information is nearly impossible due to the limited resolution of images. Therefore audio plays a significant role in this application. Nevertheless, our model struggles to capture these subtle movements. We believe this issue primarily stems from two factors: 1). the different range of motion creates an imbalance in the loss function, and 2). the audio representation is insufficient. One possible solution is to separate the motions of the right hand and left hand to generate distinct audio representations, for example, associating right-hand motion with a tempogram and left-hand motion with a spectrogram.}

\textcolor{blue}{The second case involves errors caused by inaccurate 2D estimation, as illustrated in Fig.~\ref{fig:Failure2}. Our architecture outputs full frames and our final refinement module concentrates on ensuring temporal consistency between frames, which demonstrate greater robustness compared to others, as shown in Fig.~\ref{fig:youtube_1}. However, our model still struggles from noisy 2D inputs, as it relies on an uplifting method for depth estimation. Since audio is not constrained by body structure, one possible solution is to explore the use of a human body parametric model for audio-to-pose estimation similar to the approach described in  ~\cite{liNIKINeuralInverse2023}.}


\begin{table}[t]
    \caption{\textcolor{blue}{Complexity analysis results with average performance scores.}} 
    \centering
    \resizebox{0.7\columnwidth}{!}{
    \begin{tabular}{l |c|c|c|c}
        \Xhline{1pt}
        \textbf{Method}& \textbf{\# Params} & \textbf{MPJPE} $\downarrow$ & \textbf{P-MPJPE} $\downarrow$  & \textbf{MPJAE} $\downarrow$ \\
        \hline
        PoseFormerV2 (T=81)~\cite{zhaoPoseFormerV2ExploringFrequency2023} & 	3.2 M & 50.16 &	29.85 &	5.16 \\
        STCFormer (T=81) ~\cite{tang3DHumanPose2023} & 4.7 M & 50.51 &	30.05  &13.38	\\
        MixSTE (T=243) ~\cite{zhangMixSTESeq2seqMixed2022}  & 33.8 M & 51.81 & 34.31 & 	3.39	\\
        MixSTE Light (T=243)~\cite{zhangMixSTESeq2seqMixed2022} &	2.2 M & 71.42 &	47.11 &	2.47 \\
        \hline 
        \AlgName \ without audio \ (Ours) (T=90) & 1.3 M & 49.02 &	27.85 &	1.73\\	
        \AlgName \ (Ours) (T=90, A=100)  &	4.6 M & 44.46 &	25.49 &	1.59 \\
        \AlgName \ (Ours) (T=90, A=300) & 4.8 M & 44.03 &	25.99 &	1.59 \\
        \Xhline{1pt}
    \end{tabular}
    }
    \label{tab:abl_loss}
\end{table}

\begin{figure}[h]
	\centering
	\includegraphics[width=0.85\linewidth]{fig/Tempo.pdf}
	\caption{
	    Qualitative result of tempogram estimation. The top row is the ground truth and the bottom row is the prediction from the estimated 3D pose.
	}
	\label{fig:tempo}
    % \vspace{-5mm}
\end{figure}


\begin{figure}[t]
	\centering
	\includegraphics[width=0.85\linewidth]{fig/Audio_Feature.png}
        \vspace{-2mm}
	\caption{
	    Visualization of input raw audio and computed features: Onset strength and peaks from envelope, Chroma energy normalized (CENS) and Mel-Frequency Cepstral Coefficients (MFCCs). We computed the features using the audio and music process toolbox Librosa~\cite{librosa}. 
	}
	\label{fig:audio}
    % \vspace{-5mm}
\end{figure}

\begin{figure}[h]
	\centering
	\includegraphics[width=0.9\linewidth]{fig/VioDat_result.pdf}
	\caption{
	    \textcolor{blue}{Qualitative results, tested on \DataName \ P08C02T31 with one second intervals (30 FPS).}
	}
	\label{fig:viodat_rsult}
    % \vspace{-5mm}
\end{figure}
\begin{figure}[h]
	\centering
	\includegraphics[width=0.9\linewidth]{fig/trajectory_full.pdf}
	\caption{
	    Predicted right wrist trajectories (red line) and the ground truth 3D trajectories (green line) after Procrustes projection for better comparison. Each graph contains 90 frames (3 second). The top three rows depict simple trajectories from P05C01T40, while the bottom three rows feature complex trajectories from P08C02T31. We highlight notable points as blue circle. To analyze violin bowing motion, accurately estimating wrist motion is important.
	}
	\label{fig:trajectory}
    % \vspace{-5mm}
\end{figure}

\begin{figure}[t]
	\centering
	\includegraphics[width=0.9\linewidth]{fig/youtube2.pdf}
	\caption{
	    \textcolor{blue}{Qualitative results, tested on YouTube video, are highlighted with an orange circle to emphasize the main points. From the input video, we infer that the right arm is positioned higher than shoulder level. However, \AlgName \ without audio cannot track these dynamics as effectively as \AlgName \ with audio does.}
	}
	\label{fig:youtube_2}
    % \vspace{-5mm}
\end{figure}

\begin{figure}[h]
	\centering
	\includegraphics[width=0.9\linewidth]{fig/youtube1.pdf}
	\caption{
	    \textcolor{blue}{Qualitative results, obtained from testing on a YouTube video, show that OpenPose incorrectly estimates keypoints at Frames 206 and 208. These noisy frames significantly impact the performance of both STCFormer and MixSTE.}
	}
	\label{fig:youtube_1}
    % \vspace{-5mm}
\end{figure}

\begin{figure}[h]
	\centering
	\includegraphics[width=0.9\linewidth]{fig/Vibrato.png}
	\caption{
	    \textcolor{blue}{Failure case 1: Vibrato. Green keypoints denote ground truth and blue keypoints represent its prediction. Although the ground truth hand exhibits slight movements due to the vibrato, the prediction keypoints remain static. }
	}
	\label{fig:Vibrato}
    % \vspace{-5mm}
\end{figure}
\begin{figure}[h]
	\centering
	\includegraphics[width=0.9\linewidth]{fig/Failure2.png}
	\caption{
	    \textcolor{blue}{Failure case 2: Estimation from noisy 2D input.}
	}
	\label{fig:Failure2}
    % \vspace{-5mm}
\end{figure}

\section{Limitations}
\textcolor{blue}{The VioPose dataset did not undergo any augmentation. In future research, enhancing the dataset through visual and audio data augmentation techniques could yield improved results with better generalization.}

\textcolor{blue}{We presume that the violinists possess a certain level of playing expertise. Random or unstructured manipulation of the bow on the violin typically does not generate audio of relevance for our downstream tasks. Consequently, outcomes are likely to be inferior in such instances.}

\textcolor{blue}{In the domain of violin playing, there exists an imbalance in the distribution between large and small motions. While the VioDat dataset has considerable variety and diversity, it inherits this inherent domain limitation. Notably, movements such as Detache involve slower, more prolonged actions, constituting large motions, whereas subtle techniques like tremolo entail quicker, smaller motions. As a result, the dataset exhibits an imbalance, with models demonstrating superior performance on tasks involving large motions but encountering challenges when handling subtle motions.}

\textcolor{blue}{The current model was trained using data from four camera angles, each paired with its respective audio. However, a limitation arises when the audio source and camera are not closely aligned, leading to decreased model performance. Surprisingly, the model seems to have learned to account for factors like distance, direction, and room geometry in the audio. To address this, future work should incorporate data augmentation techniques. While our focus was on pose estimation for consumer devices like smartphones, tablets, and laptops, augmentations could enhance generalization. For instance, swapping audio with cameras or modulating audio to simulate different room geometries could be explored.
}


% \begin{table*}[ht]
%     \caption{Full body estimation results}
%     \centering
%     \begin{tabular}{l|c c | c c }
%          \Xhline{1pt}
%          \multicolumn{1}{l|}{\textbf{Tested on \DataName}}& \multicolumn{2}{c|}{\textbf{Left Upper Body}} & \multicolumn{2}{c}{\textbf{Right Upper Body}} \\
%          \hline
%          \textbf{Method}  & \textbf{Elbow} & \textbf{Wrist}
%            & \textbf{Elbow} & \textbf{Wrist} \\
%          \hline
%         \multicolumn{5}{c}{\textbf{Trained on Full Body}}\\
%          \hline
%         PoseFormerV2 & 55.48 (+10.11) & 74.41 (+7.1) & 79.51 (+28.53) & 75.85 (+20.22)  \\
%         MixSTE & 54.40 (-1.43) & 77.99 (+11.66) & 59.83 (+10.51) & 68.36 (+10.55)  \\
%         \hline
%         \AlgName \ (T=90, A=300) & 52.96 (+6.9) & 71.51 (+9.41) & 60.90 (+17.2) &	61.39 (+14.99) \\
%          \Xhline{1pt}
%         \multicolumn{5}{c}{\textbf{Trained on Upper Body}}\\
%          \hline
%         PoseFormerV2 & 45.37 & 67.31 & 50.98 & 55.63 \\
%         MixSTE & 55.83 & 66.33 & 49.32 & 57.81 \\
%         \hline
%         \AlgName \ (T=90, A=300) & 46.55 & 49.49 & 35.82 & 36.02\\
        
%          \Xhline{1pt}
%     \end{tabular}
%     \label{tab:abl}
%     \vspace{-4mm}
% \end{table*}


\begin{table*}[ht]
    \caption{\textcolor{blue}{Full body estimation results}}
    \centering
    \begin{tabular}{l|c c | c c }
         \Xhline{1pt}
         \multicolumn{1}{l|}{\textbf{Tested on \DataName}}& \multicolumn{2}{c|}{\textbf{Left Upper Body}} & \multicolumn{2}{c}{\textbf{Right Upper Body}} \\
         \hline
         \textbf{Method}  & \textbf{Elbow} & \textbf{Wrist}
           & \textbf{Elbow} & \textbf{Wrist} \\
         \hline
        \multicolumn{5}{c}{\textbf{Trained on Full Body}}\\
         \hline
        PoseFormerV2 & 55.48 (+10.11) & 74.41 (+7.1) & 79.51 (+28.53) & 75.85 (+20.22)  \\
        MixSTE & 54.40 (-1.43) & 77.99 (+11.66) & 59.83 (+10.51) & 68.36 (+10.55)  \\
        \hline
        \AlgName \ (T=90, A=300) & 52.96 (+6.9) & 71.51 (+9.41) & 60.90 (+17.2) &	61.39 (+14.99) \\
         \Xhline{1pt}
        \multicolumn{5}{c}{\textbf{Trained on Upper Body}}\\
         \hline
        PoseFormerV2 & 45.37 & 67.31 & 50.98 & 55.63 \\
        MixSTE & 55.83 & 66.33 & 49.32 & 57.81 \\
        \hline
        \AlgName \ (T=90, A=300) & 46.55 & 49.49 & 35.82 & 36.02\\
        
         \Xhline{1pt}
    \end{tabular}
    \label{tab:fullbody}
    \vspace{-4mm}
\end{table*}

\begin{table*}[h]
    \centering
    \caption{\textcolor{blue}{In-the-wild test result. Separate novice participants and intermediate participant (P20)}}
    \begin{tabular}{l|cc|cc}
        \Xhline{1pt}
        \textbf{Tested on In-the-wild}& \multicolumn{2}{c|}{\textbf{Only P20}} & \multicolumn{2}{c}{\textbf{W/O P20}} \\
        \hline
         \textbf{Openpose Input} &\textbf{P-MPJPE} & \textbf{P-MPJAE}&\textbf{P-MPJPE} & \textbf{P-MPJAE} \\
        \hline
        \AlgName W/O Audio & 30.84 &	1.29&	48.34 &1.23 \\
        \AlgName  & 25.23&	1.39&	44.11&	1.3 \\
        \Xhline{1pt}
    \end{tabular}
\end{table*}


\begin{table*}[h]
    \centering
    \caption{\textcolor{blue}{In-the-wild test result with ground truth 2D input.}}
    \begin{tabular}{l|cc|cc |cc}
        \Xhline{1pt}
        \textbf{Tested on In-the-wild}& \multicolumn{2}{c|}{\textbf{Only P20}} & \multicolumn{2}{c|}{\textbf{W/O P20}} & \multicolumn{2}{c}{\textbf{Average}}\\
        \hline
         \textbf{Ground Truth Input} &\textbf{P-MPJPE} & \textbf{P-MPJAE} &\textbf{P-MPJPE} & \textbf{P-MPJAE} &\textbf{P-MPJPE} & \textbf{P-MPJAE} \\
        \hline
        PoseFormerV2 & 28.24 &	0.97 &	42.10&	0.97 & 40.19 &	0.97 \\
        STCFormer & 22.45 &	0.94 &	38.38	&0.98 & 36.18 &	0.97 \\
        MixSTE & 25.41 &	0.60 &	32.44 &	0.63 & 31.47 &	0.62 \\
        \hline
        \AlgName  & 20.22 & 	1.37&	36.08&	1.21 & 33.89 &	1.23 \\
        \Xhline{1pt}
    \end{tabular}
\end{table*}

